Mixing of Stochastic Accelerated Gradient Descent

We study the mixing properties for stochastic accelerated gradient descent (SAGD) on least-squares regression. First, we show that stochastic gradient descent (SGD) and SAGD are simulating the same invariant distribution. Motivated by this, we then establish mixing rate for SAGD-iterates and compare it with those of SGD-iterates. Theoretically, we prove that the chain of SAGD iterates is geometrically ergodic --using a proper choice of parameters and under regularity assumptions on the input distribution. More specifically, we derive an explicit mixing rate depending on the first 4 moments of the data distribution. By means of illustrative examples, we prove that SAGD-iterate chain mixes faster than the chain of iterates obtained by SGD. Furthermore, we highlight applications of the established mixing rate in the convergence analysis of SAGD on realizable objectives. The proposed analysis is based on a novel non-asymptotic analysis of products of random matrices. This theoretical result is substantiated and validated by experiments.

==> backup/introduction.tex <==
\section{Introduction}


\section{Preliminaries}
\subsection{Assumptions on the data}
\subsection{Gaussian inputs}
\subsection{Rotation of symmetric random variables*}

\section{Acceleration in realizable case}
\subsection{Results on 2d Gaussian}
\subsection{Results on d Gaussian}
\subsection{Results on d symmetric*}
\subsection{Comparison: why Gaussian is not easy?}
\subsection{Proof sketch}

\section{Acceleration in Markov chain}
\subsection{Stochastic optimization and Markov-Chain}
\subsection{Invariant distribution}
\subsection{Acceleration of discrete Markov Chains}
\subsection{Acceleration of continuous Markov Chains}

\section{Experiments} 
\subsection{Least-squares: Gaussian input, non-Gaussian inputs, real datasets}
\subsection{Logistic-regression: Gaussian input, non-Gaussian inputs, real datasets }





\subsection{Least squares regression}
Let's consider least-squares regression, namely the following minimization   
\begin{align}
   \arg \min_\w \left( \hat{f}(\w) = \frac 12 \E_{\z} \|y-\w^\top \x \|^2 \right), \quad \z:= (\x,y) \sim \P,
\end{align}
where $\x \in \R^d$ is the input variable the  and $y \in \R$ is the response variable. We can equivalently minimize
\begin{align} \label{eq:f}
    f(\w) = \frac{1}{2} \w^\top \cov \w - \E \left[ y \x^\top \w \right], \quad \cov := \E\left[ \cov \right]  
\end{align}
The gradient and stochastic gradient of the above objective are
\begin{align}
    \nabla f(\w) = \cov \w - \E \left[ y \x \right], \nabla f_\z(\w) = \x \x^\top \w - y\x.
\end{align}
Let $\mu = \lambda_{\min}(\cov)$ and $L=\lambda_{\max}(\cov)$. The condition number of the matrix $\cov$, denoted by $\kappa=L/\mu$, determines the convergence of GD on $f$. GD enjoys a linear convergence of $(1-c/\kappa)$ on $f$. %Acceleration methods such as Heavy ball method and Nesterov's acceleration  improves this convergence rate to $1-c\sqrt{1/\kappa}$\footnote{$c$ denotes any constant independent of $\cov$.}.Yet, it is not clear whether these method are advantageous in stochastic optimization. %Recently, \cite{dieuleveut2017harder,jain2018accelerating} have motivated using acceleration techniques for stochastic optimization.   
%Here, we investigate the acceleration techniques for stochastic optimization in a simplified setting. 
\subsection{Acceleration for stochastic optimization}
 \paragraph{Heavy ball (HB) method} HB method is an accelerated method designed particularly for \textbf{quadratic} convex objectives. This method optimizes $f$ through the following recurrence: \begin{align}
      \w_{n+1} = \w_n - \gamma \nabla f(\w_n) + \beta (\w_n - \w_{n-1}), \quad \w_1 = \w_0.
 \end{align}
 For $\beta = (\kappa-1)/(\kappa+1)$ and $\gamma=\min\{4/(L+\mu)^2,1/L\}$, HB converges linearly to the minimizer $\w^*$ (of $f$) \cite{jung2017fixed}:  
 \begin{align}
     \| \w_n - \w^* \|^2 \leq C(\kappa)n \left(\frac{\sqrt{\kappa}-1}{\sqrt{\kappa}+1}\right)^n \| \w_0 - \w^*\|^2,
 \end{align}
 where $C(\kappa) = 4 (2+2\beta^2+4\gamma)/(\beta^{-1}) $
 (See \cite{recht2010}.).
 \paragraph{Nesterov Acceleration}
 Although HB successfully accelerates the convergence of GD on convex quadratics, there is no global convergence guarantee for this method on non-quadratic functions \footnote{There are global convergence guarantees for HB but these guarantees does not show any acceleration compared to GD.}. Nesterov adapted HB to reach a globally accelerated rate for convex and strongly convex objectives. Nesterov's proposal is based on two sequence of iterations as 
 \begin{align}
     \w_{n+1} & = \v_n - \gamma \nabla f(\v_n) \\ 
     \v_{n+1} & = \w_{n+1} + \beta (\w_{n+1}- \w_n)
 \end{align}
 We can show that $\w_{n+1}$ converges to $\w^*$ as 
 \begin{align}
     f(\w_{n}) - f(\w^*) \leq (L+\mu) \exp(-(n-1)/\sqrt{\kappa})\| \w_0 - \w^*\|^2 
 \end{align}
 where $\mu$ is strong convexity constant and $L$ is the smoothness parameter \footnote{There is summarized proof for the above result in  \href{https://blogs.princeton.edu/imabandit/2014/03/06/nesterovs-accelerated-gradient-descent-for-smooth-and-strongly-convex-optimization/}{this blog}.)}. The key element in the Nesterov's modification is extrapolation. To observe that, we swap updates as
 \begin{align}
 \v_{n} & = \w_{n} + \beta (\w_{n}- \w_{n-1}) \\ 
 \w_{n+1} & = \v_n - \gamma \nabla f(\v_n)
 \end{align}
 Then we combine the above two sequences in one: 
 \begin{align}
     \w_{n+1}= \w_{n+1/2} - \gamma \nabla f(\w_{n+1/2}), \quad  \w_{n+1/2} := \w_{n} + \beta (\w_{n}- \w_{n-1})
 \end{align}
 As we see, the gradient is evaluated at $\w_{n+1/2}$ obtained by the extrapolation $\w_{n+1/2}$. 
 
\paragraph{Stochastic acceleration schemes}
Replacing the gradient with a stochastic approximation of gradient in HB and Nesterov's acceleration method leads to stochastic HB (SHB) and stochastic Nesterov's acceleration (SNA): 
\begin{align} 
\text{SHB:} & \w_{n+1} = \w_n - \gamma \nabla f_\z(\w_n) + \beta (\w_{n} - \w_{n-1}) \\ 
\text{SNA:} & \w_{n+1} = \w_{n+1/2} - \gamma \nabla f_\z(\w_{n+1/2}), \quad \w_{n+1/2}:=\w_{n} + \beta (\w_{n}- \w_{n-1})
\end{align} 
What is the difference between SGD and the above accelerated stochastic methods? How the noise of stochastic approximation interacts with the momentum term? Can we robustify these method against the noise of stochastic approximation? These are questions that we want to investigate here.
\paragraph{Gaussian input}
 We repeatedly use the following result on Gaussian inputs. 
\begin{lemma} \label{lemma:gaussianity_consequence} 
Suppose that $\x$ is drawn from a zero-mean multivariate normal distribution, i.e. ${\x \sim \N(0,\cov)}$, then the following holds for every matrix $\M$: 
\begin{align} \label{eq:gaussianity_consequence}
    \E \left[ \x \x^\top \M \x \x^\top \right] = 2 \cov \M \cov + \langle \M, \cov \rangle \cov 
\end{align}
where $ \langle \M, \cov \rangle$ is the inner product of vectorized $\M$ and $\cov$.
\end{lemma}
\begin{proof} 
Let $\A$ be the desired matrix as 
\begin{align} \label{eq:a_matrix}
\A := \E \left[ \x \x^\top  \M \x \x^\top  \right].
\end{align} 
Element $\A_{ij}$ can be computed as 
\begin{align}
    \A_{ij} & = \E \left[ \x_i \x_j \sum_{k,l}  \x_l \M_{lk} \x_{k}  \right] \\ 
    & = \sum_{lk} \E \left[ \x_i \x_j \x_l \x_k \right]  \M_{lk}.
\end{align}
Since $\x$ is Gaussian, we can compute its 4th order statistics using the 2nd order statistics:
\begin{align}
    \A_{ij} = \cov_{ij} \left( \sum_{kl} \cov_{kl} \M_{kl} \right) + 2 \sum_{lk} \cov_{ik}  \M_{kl} \cov_{lj} 
\end{align}
Writing the above equation in the matrix equivalent form concludes the proof: 
\begin{align} \label{eq:E_y_mn_y}
    \A := \langle \cov, \M \rangle \cov + 2 \cov   \M \cov  
\end{align}

\end{proof}




   


==> backup/mc.tex <==
\section{Markov chain and stochastic optimization}
\subsection{SGD and Markov chains}
\paragraph{SGD and Markov chains} Recall SGD iterates on objective $f$ as 
\begin{align}
    \w_{n} = \w_n - \gamma \nabla f_\z(\w), \quad \nabla f_\z(\w) = \x\x^\top \w - \y \x 
\end{align}
Sequence $\{\w_k\}_{k=1}^n$ makes a homogeneous Markov chain on $\R^d$ convergent to a unique stationary distribution. Bridging SGD with Markov chain allows us not only understand the behaviour of SGD better but also it is useful in designing new optimization techniques~\cite{dieuleveut2017bridging}.  For example, stochastic averaging of iterates can be very well-analyzed by tools from Ergodicity theory (See \cite{babichev2018constant} for an overview). Here, we particularly focus on the convergence of constant stepsize SGD to a stationary distribution. Later, we will show the applications of the convergence of SGD to its stationary distribution. 
\paragraph{Convergence to the stationary distribution for SGD: A coupling approach}
Here, we prove the convergence of SGD to an stationary distribution --independent from its initialization scheme. Our prove is based on the result of ~\cite{dieuleveut2017bridging}.
Let's consider the space of probability measures on $\R^d$ endowed with Wasserstein 2 metric $W$ defined as 
\begin{align}
    (W_2(\mu,\nu))^2 = \inf_{(\v,\w) \in L(\mu,\nu)} \E \left[ \| \v - \w \|^2 \right]  
\end{align}
We know that the space of probability measure with Wasserstein 2 metric is complete. Consider two different sequences of SGD starting at random, namely  
\begin{align}
    \w_{n+1}^{(1)} &= \w_{n}^{(1)} - \gamma \nabla f_{\z_n}(\w_{n}^{(1)}), \quad  \w_0^{(1)} \sim \mu_0 \\ 
    \w_{n+1}^{(2)} &= \w_{n}^{(2)} - \gamma \nabla f_{\z_n}(\w_{n}^{(2)}), \quad  \w_0^{(2)} \sim  \nu_0
\end{align}
Remarkably, we the used the same $\z_n$ in both of updates. Let consider the compact notation $\Delta \w_{n} := \w_n^{(1)} - \w_n^{(2)}$.  
This notation and SGD updates yields 
\begin{align} 
\Delta \w_{n+1} = \left( \I - \gamma \x_n \x^\top_n \right) \Delta \w_{n} = \B_n \Delta \w_{n} 
\end{align} 
where $\B_n$ is the product of random matrices in Eq.~\eqref{eq:SGD_iterates}. According to Theorem 4.1. of \cite{villani2008optimal}, there are a couple of random variables $\w_0$ and $\v_0$, independent from $\{\z_i\}_{i=1}^n$s, such that 
\begin{align} \label{eq:w_match_0}
    (W_2(\nu_0,\mu_0))^2 = \E \| \w_0 - \v_0 \|^2
\end{align}
Let $\mu_n$ and $\nu_n$ denote the probability laws of random variables $\w_{n}^{(1)}$ and $\w_{n}^{(2)}$ (starting from $\w_0$ and $\v_0$). Then according to the definition of the Wasserstein distance, we have 
\begin{align}
    (W_2(\mu_n,\nu_n))^2  & \leq \E \left[ \| \w_n^{(1)} - \w_n^{(2)} \|^2  \right]  \\ 
    & = \E \left[ \| \Delta \w_n \|^2 \right] \\ 
    & = (\Delta \w_0)^\top \E \left[ \B_n^\top \B_n \right] (\Delta \w_0) \\ 
    & \leq  \E \| \Delta \w_0 \|^2 \| \E \left[ \B_n^\top \B_n \right] \|  \\ 
    & \stackrel{\eqref{eq:w_match_0}}{=} (W_2(\mu_0,\nu_0))^2 \| \E \left[ \B_n^\top \B_n \right] \| \\ 
    & \leq (W_2(\mu_0,\nu_0))^2 \tr( \E \left[ \B_n^\top \B_n \right]) \\ 
    & \stackrel{\eqref{eq:eigenvalues_sgd}}{\leq } (W_2(\mu_0,\nu_0))^2 \| \C^n \ones \|, \quad \text{Lemma~\ref{lemma:sgd}}\\
    & \leq (W_2(\mu_0,\nu_0))^2 \| \C \|^n d
\end{align}
A reasonable choice of the stepsize gaurantees $\| \C \| < 1$ holds in the above inequality concludes an exponential convergence rate in $W_2$. This result is sufficient to conclude that $\mu_n$ is Cauchy. The completeness of the space concludes that $\mu_n$ converges to a unique stationary distribution~\footnote{This result can be extended to an arbitrary strongly convex function under weak assumptions on stochastic gradient (see Proposition 2. of \cite{dieuleveut2017bridging}).}. Therefore, the convergence analysis of the realizable case in Lemma~\ref{lemma:sgd} is equivalent to establishing a rate on the convergence of SGD to its stationary distribution. We can extend this result to stochastic accelerated methods. 
\subsection{Acceleration of discrete-state Markov chains}
Consider a discrete state Markov chain with $d$ statates. Transition matrix 


==> backup/realizable-leastsquares.tex <==
\section{Acceleration in Realizable settings}
We turn our focus into realizable least-squares where there is a $\w^*$ generating the response as $y = \x^\top \w^*$.  This setting is recently motivated by over-parameterization models of neural networks \cite{schmidt2018fast,jain2018accelerating}. We will further motivate this setting from Markov chain perspective. 
 
\subsection{Extra extrapolation}
Throughout the rest of the manuscript, we assume that the input is drawn from a zero-mean multivariate normal distribution, i.e. $\x \sim \N(0,\cov)$. Let's define extra-extrapolated stochastic gradient descent (EESGD) as 
\begin{align} 
    \w_{n+1} = \w_n + \beta (\w_n - \w_{n-1}) - \gamma \nabla f_\z(\w_n + \alpha(\w_{n}-\w_{n-1})
\end{align}
where $\beta<1$ but $\alpha$ can be greater than 1. We observe that  stochastic HB and stochastic Nesterov's acceleration  requires a small momentum constant $\beta$ to avoid divergence caused by stochasticity of the gradient estimate. A large $\alpha$ allows us to use relatively high $\beta$ in that reach an acceleration. Results in Figure~\ref{fig:extrapolation_result} compare the convergence of SHB, SNA and the proposed extra-extrapolated stochastic gradient descent. Note that we search over $\gamma$ and $\beta$ for this result and it is not clear what is the best choice for stochastic optimization. A clear comparison between these method requires a theoretical justification on the convergence rate obtained by optimal parameters for each method. Indeed, we need to find the optimal $\alpha$, $\beta$, and $\gamma$ to achieve the best rate. 
%If the optimal $\alpha$ is larger than 1, then we can claim extra-extrapolation is useful in stochastic setting. But more important question is whether we can reach the same acceleration as deterministic setting, i.e. linear convergence rate $(1-\sqrt{\mu/L})$. 
\begin{figure} \label{fig:extrapolation_result}
    \centering
    \includegraphics[width=0.8\textwidth]{images/extra_extrapolation.pdf}
    \caption{Extra-extrapolation is useful in a stochastic setting. In this experiement, the horizontal axis is $\log(\| \w - \w^*\|^2)$. The input is $\x \sim N(0,\diag(\bsigma))$ where $\bsigma_i = i^{-4}$ for $i=1, \dots, 16$.}
    \label{fig:my_label}
\end{figure}
\subsection{Warm-up: convergence analysis of SGD}
To warm-up, we prove the convergence rate of SGD on Gaussian inputs. This result give us some intuitions about the noise of SGD and how it can effect the convergence in a realizable setting. Without loss of generality, we assume that $\w^* = 0$, hence 
\begin{align}
    \nabla f_\x(\w) = \x \x^\top \w. 
\end{align}
Using the stochastic gradient formulation, we derive SGD updates by product of random matrices 
\begin{align} \label{eq:SGD_iterates}
    \w_{n} = (\I - \gamma \x_n \x^\top_n) \w_{n-1} = \B_n \w_0, \quad \B_n :=\prod_{k=1}^{n} (\I - \gamma \x_k \x^\top_k)
\end{align}
Our goal is to show that $\w_n$ converges to zero, i.e. the following holds 
\begin{align}
    \lim_{n\to \infty}  \| \w_n \|^2  = 0 
\end{align}

\paragraph{Why we can assume that $\w^* =0$?}
Suppose that $\w^* \neq 0$, then stochastic gradient can be written as 
\begin{align}
     \nabla f_\z(\w) & = \x\x^\top \w - y \x \\ 
     & \stackrel{(\eta)}{=} \x \x^\top \w - \x \x^\top \w^* \\ 
     & = \x \x^\top (\w - \w^*) 
\end{align}
 In $\eta$, we do exploit the realizability as $y = \x^\top \w^*$. Now, we can write SGD updates as 
 \begin{align}
     \w_{n+1} - \w^* = (I - \gamma \x_n\x^\top_n)(\w_n - \w^*) 
 \end{align}
 Therefore, we can replace $\w_n$ (and $\w_{n-1}$) in Eq.~\eqref{eq:SGD_iterates} by $\w_n - \w^*$ (and $\w_{n-1} - \w^*$) and all the rest of analysis still holds. 


We can prove the above result in two ways: (i) using existing result on product of random matrices or (ii) compute $E\left[ \B_n^\top \B_n\right] $ and prove its eigenvalues tends to zero for large $n$. Product of random matrices studies the asymptotic grow rate of $\| \B_n \|$ by showing that  
\begin{align}
    \lim_{n\to \infty} \frac 1n \log(\|\B_n \|) = \lambda_1
\end{align}
holds with probability one. $\lambda_1$ is the top Lyapunouv exponent of the product of the random matrices (You can find a very short proof of the above result in Example 7.5.1. of \cite{durrett2010probability} which is based on subadditive Ergodic theorem. \cite{bougerol2012products} is an introductory lecture on product of random matrices.).
The later approach (ii) allows us to reach a non-asymptotic result (for finite $n$), while the existing result on product of random matrices all are asymptotic. To show the desired norm decay, we need to bound the top eigenvalue of $\B_n^\top \B_n$. 
\begin{align}
    \E \| \w_n \|^2  = \w_0^\top \E \left[ \B_n^\top \B_n \right] \w_0 
\end{align}
To compute the above expectation, we first reverse the indexing, namely we assume that $\B_n = (\I-\gamma \x_1 \x_1^\top) \dots (\I - \gamma \x_n \x_n^\top)$. Then, we make the following recurrence 
\begin{align}
    \E \left[ \B_{n+1}^\top \B_{n+1} \right] &= \E \left[ (\I - \gamma \x \x^\top) \B_n^\top \B_n (\I - \gamma \x \x^\top) \right] \\ 
    &= \E \left[ \B_n \B_n^\top \right]  - \gamma \cov \E \left[ \B_n^\top \B_n \right] - \gamma \E \left[ \B_n^\top \B_n \right] \cov + \gamma^2 \E \left[ \x \x^\top \B_n^\top \B_n \x \x^\top \right]\nonumber \\ 
    & \stackrel{\eqref{eq:gaussianity_consequence}}{=} (\I - \gamma \cov) \E \left[ \B_n \B_n^\top \right] (\I - \gamma \cov) + \gamma^2 \cov \E \left[ \B_n^\top \B_n \right] + \langle \cov, \E \left[ \B_n^\top \B_n \right] \rangle \cov \label{eq:E_BB_recursive}
\end{align}
The above recurrence allows us to track the expectation $\E\left[ \B_n^\top \B_n \right]$ in a closed-form. The next lemma tracks eigenvalues and eigenvectors of  this matrix separately \footnote{We established a similar result for PCA problem during my visit at INRIA, but we later found a better way to solve our question. The analysis of the Gaussian case gave us very helpful intitutions there. }.
\begin{lemma} \label{lemma:sgd}
    Consider the following eigenvalue decomposition for the covariance matrix of the input $\cov = \U \diag(\bsigma)\U^\top$. If $\x \sim \N(0,\cov)$ then 
    \begin{align}
        \E \left[ \B_n^\top \B_n \right] = \U \diag(\blambda_n) \U^\top 
    \end{align}
    where 
    \begin{align} \label{eq:eigenvalues_sgd}
        \blambda_n = \C^n \ones, \quad \C := (\I - \gamma \diag(\bsigma))^2 + \gamma^2 \diag(\bsigma)^2 + \gamma^2 \bsigma \bsigma^\top 
    \end{align}
\end{lemma}
\begin{proof}
Our proof is based on induction: supposing the above result holds for $n$, we prove that it holds for $n+1$. 
\begin{multline}
    \E \left[ \B_{n+1} \B_{n+1}^\top \right] \stackrel{\eqref{eq:E_BB_recursive}}{=}  \U  \left(  (\I-\gamma \diag(\bsigma)) \diag(\blambda_n) (\I - \gamma \diag(\bsigma)) \right) \U^\top 
    \\ +  \gamma^2 \U \left( \diag(\bsigma) \diag(\blambda_n) \diag(\bsigma) + \langle\bsigma,\blambda_n\rangle \diag(\bsigma) \right) \U^\top
\end{multline}
From the above equation, we can prove that $\blambda_{n+1}$ is obtained by the following affine transformation of $\blambda_n$: 
\begin{align}
     \blambda_{n+1} = \C \blambda_{n}
\end{align}
where $\C$ is the matrix in Eq.~\eqref{eq:eigenvalues_sgd}. This result conclude our induction. 
\end{proof}
According to the result of last lemma, SGD with stepsize $0.5/(L+\tr[\cov])$ linearly converge to $\w^* =0$ with rate $1-0.5\mu/(L+\tr[\cov])$. The rate of convergence is slightly worst than the convergence rate of gradient descent, which is $1-\mu/L$.


\subsection{Convergence analysis for accelerated stochastic optimization}
Recall our general stochastic accelerated method as 
\begin{align}
    \w_{n+1} = \w_n + \beta (\w_n - \w_{n-1}) - \gamma \nabla f_\z(\w_n + \alpha(\w_{n}-\w_{n-1}))
\end{align}
Setting $\alpha =0$ in the above equation recovers SHB method and $\alpha = \beta$ reduces to Stochastic Nestrov's acceleration method. Our question is: is there any choice for parameters $\alpha$, $\beta$ and $\gamma$ such that the above method improves upon the established convergence rate of SGD in the last section. To address this question, we first write the update in the following linear recurrence: 
\begin{align}
    \begin{bmatrix} 
    \w_{n+1} \\ 
    \w_{n}
    \end{bmatrix} = \A_n \begin{bmatrix} 
    \w_{n} \\ 
    \w_{n-1}
    \end{bmatrix}, \quad \A_n := \begin{bmatrix} 
    (1+\beta) \I- (1+\alpha) \gamma \x_n\x^\top_n & \alpha \gamma \x_n \x^\top_n - \beta \I \\ 
    \I & 0 
    \end{bmatrix}
\end{align}
We write matrix $\A_{n+1}$ as 
 \begin{align} \label{eq:An_decomposition}
     \A_{n+1} = \A -\gamma 
     \epsilon, \quad \epsilon := \begin{bmatrix} 
     (1+\alpha) \Delta & -\alpha\Delta \\ 
     0 & 0 
     \end{bmatrix}, \Delta :=(\cov - \x \x^\top)
 \end{align}
 where $\E \left[ \epsilon \right] = 0$ and matrix $\A$ is 
 \begin{align}
     \A = \begin{bmatrix} 
     \A_1 & \A_2 \\ 
     \I & 0 
     \end{bmatrix}, \A_1 := (1+\beta)\I - \gamma (1+\alpha) \cov, \A_2 := \alpha \gamma \cov - \beta \I  
 \end{align}
 The above decomposition allows us to analyze the covariance term induced by the noise separately.
Similar to our analysis for SGD, we aim at tracking matrix $ \M_n := \E \left[\A_n^\top \dots \A_1^\top \A_1 \dots \A_n \right] $ in a closed form. The next lemma provides a recurrence that later will be used to track the desired matrix.   
\begin{lemma} 
Suppose $\x \sim \N(0,\cov)$. Consider the following block structure: 
\begin{align}
     \E \left[ \M_n \right] = \begin{bmatrix} 
      \M_1 & \M_2 \\ 
      \M_2 & \M_3 
     \end{bmatrix}.
\end{align}
Then matrix $\E\left[ \M_{n+1} \right]$ can be decomposed as
\begin{align} \label{eq:E_nplus_expansion_result}
    \E \left[ \M_{n+1} \right] = \A^\top  \E \left[\M_n \right]\A + \gamma^2 \underbrace{\begin{bmatrix} (1+\alpha)^2 \K &  -\alpha(1+\alpha) \K \\
 -\alpha (1+\alpha) \K  & \alpha^2 \K 
 \end{bmatrix}}_{\text{due to the noise}}
\end{align}
where  \begin{align}
    \K := \cov \M_1 \cov + \langle \cov,\M_1 \rangle \cov.
\end{align}
\end{lemma} 
\begin{proof}
 Using the decomposition of matrix $\A_n$ in Eq.~\eqref{eq:An_decomposition}, we expand the expectation as  
 \begin{align}\label{eq:M_nplus}
     \E \left[ \M_{n+1} \right] & = \E \left[\A_{n+1}^\top  \M_n \A_{n+1}  \right] \\   
     & = \A^\top  \E \left[\M_n \right]\A + \gamma^2  \E \left[ \epsilon^\top  \M_n \epsilon \right] 
 \end{align}

We compute 2nd term (induced by the noise) 
\begin{align} \label{eq:variance_noise}
    \E \left[ \epsilon^\top  \M_n \epsilon \right]  = \begin{bmatrix} 
    (1+\alpha)^2 \Delta \M_1 \Delta & -\alpha (1+\alpha) \Delta\M_1 \Delta \\ 
    -\alpha (1+\alpha) \Delta\M_1 \Delta & \alpha^2 \Delta \M_1 \Delta
    \end{bmatrix} 
\end{align}
Using lemma~\ref{lemma:gaussianity_consequence} on Gaussian inputs, we have 
\begin{align}
    \E \left[ \Delta \M_1 \Delta \right] =  \cov \M_1 \cov + \langle \M_1,\cov \rangle \cov 
\end{align}
Replacing this result into Eq.~\eqref{eq:M_nplus} concludes the proof.
\end{proof}
The first term in Eq.~\eqref{eq:E_nplus_expansion_result} is the update with exact gradient and the 2nd term is caused by the noise of the stochastic gradient.  
Using the above result, next corollary proves that $\E\left[ \M_n \right]$ can be computed through a linear fixed point iteration.
\begin{corollary} 
Suppose that $\x \sim N(0,\cov) $ where $\cov = \U \diag(\bsigma) \U^\top$; then 
\begin{align}
     \E \left[ \M_n \right] = \begin{bmatrix} 
      \M_1 & \M_2 \\ 
      \M_2 & \M_3 
     \end{bmatrix}, \quad \M_{i} = \U \diag(\blambda_n^{(i)}) \U^\top
\end{align}
where 
\begin{align}
    \begin{bmatrix} 
    \blambda_n^{(1)} 
     \\ 
    \blambda_n^{(2)}
    \\
    \blambda_n^{(3)}
     \end{bmatrix} =
     \C^n
    \ones
\end{align}
and matrix $\C$ is 
\begin{align}
    \C & = \begin{bmatrix} \D_1^2 + (1+\alpha)^2 \K_\epsilon & 2 \D_1 & \I \\ 
     \D_1 \D_2 - \alpha(1+\alpha) \K_\epsilon& \D_2 & 0 \\ 
     \D_2^2 +\alpha^2 \K_\epsilon & 0 & 0
    \end{bmatrix}  \label{eq:C_matrix}\\ 
    \D_1 &= (1+\beta) \I - \gamma (1+\alpha) \diag(\bsigma),\\ 
    \D_2 &=  \alpha \gamma \diag(\bsigma) - \beta \I \\ 
    \K_\epsilon &= \gamma^2 \left( \diag(\bsigma)^2 +\bsigma \bsigma^\top \right)
\end{align}
\end{corollary}
\begin{proof}
  We prove the result by induction. 
  Recall matrix $\A$ with the following block structure: 
\begin{align}
     \A = \begin{bmatrix} 
     \A_1 & \A_2 \\ 
     \I & 0 
     \end{bmatrix}, \A_1 := (1+\beta)\I - \gamma (1+\alpha) \cov, \A_2 := \alpha \gamma \cov - \beta \I
 \end{align}
Indeed, $\D_i$ are the diagonal matrix of eigenvalues of matrix $\A_i$. We decompose $\E\left[ \M_n \right]$ as 
 \begin{align}
      \E \left[ \M_n \right] = \begin{bmatrix} 
      \M_1 & \M_2 \\ 
      \M_2 & \M_3 
     \end{bmatrix}, \M_i = \U \diag(\blambda_n^{(i)}) \U^\top 
 \end{align}
  Using the above expression,  
  we expand the first term in Eq.~\eqref{eq:E_nplus_expansion_result}
\begin{align}
    \A^\top \E \left[ \M_n \right] \A & = \begin{bmatrix} 
    \A_1 \M_1 \A_1 + 2\M_2 \A_1 + \M_3 & \A_1 \M_1 \A_2 + \M_2 \A_2 \\ 
    \A_2 \M_1 \A_1 + \M_2 \A_2 & \A_2 \M_1 \A_2 
    \end{bmatrix} \\ 
    & = 
    \begin{bmatrix} 
     \B_1 & \B_2 \\ 
     \B_2 & \B_3 
    \end{bmatrix} 
\end{align}
where 
\begin{align}
    \B_1 &= \U \left( \D_1^2 \diag(\blambda_n^{(1)}) + 2 \D_1\diag(\blambda_n^{(2)}) + \diag(\blambda_n^{(3)})\right) \U^\top \\ 
    \B_2 &= \U \left( \D_1 \D_2 \diag(\blambda_n^{(1)}) + \D_2 \diag(\blambda_n^{(2)}) \right) \U^\top \\ 
    \B_3 & = \U \left(  \D_2^2 \diag(\blambda_n^{(1)}) \right) \U^\top 
\end{align}
Using eigendecomposition of $\cov$ and $\M_1$, the matrix $\K$ in the noise-induced term can be written as 
\begin{align}
     \K  = \U \left(  \diag(\bsigma)^2 \diag(\blambda_n^{(1)}) + \langle \blambda_n^{(1)}, \bsigma \rangle \diag(\bsigma) \right) \U^\top
\end{align}
Putting all together, we complete the proof: 
\begin{align}
    \E \left[ \M_{n+1} \right] = \begin{bmatrix} 
    \M_{1}^+ & \M_2^+ \\ 
    \M_2^+ &  \M_3^+
    \end{bmatrix}, \quad  \M_i^+ = \U \diag(\blambda_{n+1}^{(i)}) \U^\top 
\end{align}
where 
\begin{align}
    \begin{bmatrix} 
    \blambda_{n+1}^{(1)} 
     \\ 
    \blambda_{n+1}^{(2)}
    \\
    \blambda_{n+1}^{(3)}
     \end{bmatrix} =
     \C
     \begin{bmatrix} 
    \blambda_n^{(1)} 
     \\ 
    \blambda_n^{(2)}
    \\
    \blambda_n^{(3)}
     \end{bmatrix}
\end{align}
where matrix $\C$ is those of Eq.~\eqref{eq:C_matrix}. 
The above results concludes our induction. 
\end{proof}
Using the result of last corollary, we only need to analyze eigenvalues of matrix $\C$ to prove the convergence of stochastic accelerated methods. We highlighted the noise effect with the subscript $\epsilon$. We clearly see the effect of changing extrapolation constant $\alpha$ in matrix $\C$. If $\alpha=0$, then the noise will be applied just to $\blambda_{n+1}^{(1)}$.  For a larger $\alpha$ the noise will be distributed through all eigenvalues $\blambda_{n+1}^{(i)}$. The complex eigenvalues of matrix $\C$ can be analyze using a similar proof technique that is used in Heavy ball analysis. Here is our plan for computing eigenvalues of $\C$. 
\begin{itemize}
    \item We first establish a bound on eigenvalues of matrix $\K_\epsilon$. Note that this matrix is obtained by a rank one modification of a diagonal matrix, hence we can easily bound its spectrum. 
    \item Then we use the rearrangement of row and columns of $\C$ to make it block diagonal. In this way, we need to analysis eigenvalues of $3\times 3$ matrices to derive eigenvalues of $\C$.
\end{itemize}

\subsection{Spectral radius analysis: 2D case} 
In the rest of the document, we establish a bound on the spectral radius of $\C$. Recall matrix $\C$ formulation:
\begin{align}
    \C : = \begin{bmatrix} \C_1 & 2 \D_1 & \I \\ 
     \C_2 & \D_2 & 0 \\ 
     \C_3 & 0 & 0
    \end{bmatrix}
\end{align}
where 
\begin{align}
    \C_1 & = \D_1^2 + (1+\alpha)^2 \K_\epsilon, \quad \D_1 := (1+\beta) \I - \gamma (1+\alpha) \diag(\bsigma)\\ 
    \C_2 & = \D_1 \D_2 - \alpha(1+\alpha) \K_\epsilon, \quad \D_2 =  \alpha \gamma \diag(\bsigma) - \beta  \K_\epsilon\\ \C_3 & = \D_2^2 +\alpha^2 \K_\epsilon, \quad \K_\epsilon := \gamma^2 \left( \diag(\bsigma)^2 +\bsigma \bsigma^\top \right)
\end{align}

To warm-up, we start our analysis with a 2D Gaussian input such that 
\begin{align}
    \E \left[ \x \x^\top \right] = \diag( \bsigma), \quad \bsigma :=[L, \mu]
\end{align}
where $L$ is the maximum eigenvalue of input covariance and $\mu$ is the minimum eigenvalue of the input. Our focus is on cases where $L$ is significantly larger than $\mu$, i.e. $L \gg \mu$. In this case, we can decompose $\K_\epsilon$ (the induced matrix by noise) as sum of diagonal matrices and a non-diagonal matrix: 
\begin{align}
    \K_\epsilon := \gamma^2 \left( \diag(\bsigma)^2 + \diag\left([L^2,\mu^2]\right) + \xi\right), \quad \xi = \begin{bmatrix} 
    0 &  \mu L \\ 
    \mu L & 0 
    \end{bmatrix}
\end{align}
The non-diagonal matrix $\xi$ has a bounded norm since 
\begin{align}
    \| \xi \| \leq \| \xi \|_F  \leq 2 \mu L.
\end{align}
Using the decomposition of $\K_\epsilon$, we decompose $\C$ as a perturbation of a block diagonal matrix: 
\begin{align}
    \C = \bar{\C} + \gamma^2  
    \begin{bmatrix} 
    (1+\alpha)^2 \xi & 0 & 0 \\ 
    -\alpha(1+\alpha) \xi & 0 & 0 \\ 
    \alpha^2 \xi & 0 & 0
    \end{bmatrix}
\end{align}
where matrix $\bar{C}$ is 
\begin{align}
    \bar{\C} := \begin{bmatrix} \D_1^2 + (1+\alpha)^2 \bar{\K}   & 2 \D_1 & \I \\ 
     \D_1 \D_2 - \alpha(1+\alpha) \bar{\K}& \D_2 & 0 \\ 
     \D_2^2 +\alpha^2 \bar{\K} & 0 & 0
    \end{bmatrix}, \quad \bar{\K} := 2 \gamma^2 \left( \diag(\bsigma)^2  \right)
\end{align}
Our goal is using pseudospectrum of $\C$ to bound  $\| \C^n \|$ (see~\cite{jensen09}). 
\paragraph{Background on pseudospectrum}
Pseudospectrum is mainly developed for perturbation analysis of non-hermitian matrix. Let $\sigma(\A)$ be the set of complex eigenvalues of the non-symmetric matrix $\A$; then the spectral radius of $\A$ is $\rho(\A) = \sup\{ |\z|\; | \; \z \in \sigma(\A) \}$. $\epsilon$-pseudospectrum of $\A$, denoted by  $\sigma_{\epsilon}(\A)$, is defined as 
\begin{align}
    \sigma_{\epsilon}(\A) := \sigma(\A) \cup \{ \z \in C \; | \; \| (\A - \z \I)^{-1} \| \geq 1/\epsilon \}. 
\end{align}
Pseudospectrum of $\A$ is a genealization of spectral radius for $\epsilon$-pseudospectrum as   
\begin{align}
    \rho_\epsilon(\A) = \sup\{ |\z| \; | \; \z \in \sigma(\A) \} 
\end{align}
Three key results on $\rho_\epsilon(\A)$ are presented in next three lemmas. 
\begin{lemma}[Matrix power and Pseudospectrum (Theorem 9.2\cite{jensen09})] 
The following holds for any $\epsilon$ and all $n$: 
\begin{align}
    \| \A^n \| \leq \frac{(\rho_{\epsilon}(\A))^{n+1}}{\epsilon}
\end{align}
\end{lemma}
\begin{lemma}[Robustness of Pseudospectrum (Theorem 5.12.\cite{jensen09})] 
For all matrices $\M$, the following holds 
\begin{align}
    \rho_{\epsilon}(\A + \M) \leq \rho_{\epsilon+\|\M\|}(\A)
\end{align}
\end{lemma}
\begin{lemma}[Bauer–Fike; see Thm. 5.11 of \cite{jensen09}]
Let $\A$ be a diagonalizable square matrix such that $\A = \V \Lambda \V^{-1}$. Then for $\epsilon>0$, the following holds: 
\begin{align}
    \rho_\epsilon(\A) \leq \kappa \epsilon
\end{align}
where $\kappa$ is the condition number of $\V$.
\end{lemma} 
\paragraph{Diagonalization of $\bar{\C}$}

Since matrix $\bar{\C}$ has a block diagonal structure, we can permute its rows and columns to make a block diagonal matrix as 
\begin{align}
    \Pi \bar{\C} \Pi^\top = \begin{bmatrix} 
     \M_{1} & 0&  0 & \dots & 0 \\ 
     0 & \M_{2} & 0 & \dots & 0 \\ 
     \vdots & \vdots & \vdots & \vdots & \vdots \\ 
     0 & \dots & \dots & 0 & \M_{d} 
    \end{bmatrix} 
\end{align}
where $\M_{i}$ is a $3 \times 3$ matrix as
\begin{align}
    \M_{i} := \begin{bmatrix} 
     m_1  & m_2 & 1 \\ 
    m_3 & m_4 & 0 \\ 
    m_5 & 0 & 0
    \end{bmatrix} 
\end{align}
where 
\begin{align}
    m_1 & := D_{1i}^2 + 2 (1+\alpha)^2 \gamma^2 \sigma_i^2  \\
    m_2 & := 2 D_{1i} \\ 
    m_3 & := D_{1i}D_{2i} - 2 \alpha (1+\alpha)  \gamma^2 \sigma_i^2 \\ 
    m_4 & := D_{2i} \\ 
    m_5 & := D_{2i}^2 + 2 \gamma^2 \alpha^2 \sigma_i^2
\end{align}
Given diagonalization $\M_i = \U_i \Lambda_i \U_i^\top $ , then we have
\begin{align}
     \bar{\C}  
    = 
    \V 
    \begin{bmatrix} 
    \Lambda_{1} & 0&  0 & \dots & 0 \\ 
     0 & \Lambda_{2} & 0 & \dots & 0 \\ 
     \vdots & \vdots & \vdots & \vdots & \vdots \\ 
     0 & \dots & \dots & 0 & \Lambda_{d}
     \end{bmatrix}
    \V^\top
\end{align}
where matrix $\V$ is an orthogonal matrix as 
\begin{align}
    \V := \Pi^\top 
    \begin{bmatrix}
        \U_1  & 0 & \dots \\ 
        0 & \U_2  & \dots \\ 
        \vdots & \vdots & \vdots 
    \end{bmatrix}.
\end{align}
Since $\V$ is orthogonal, its condition number is $1$. 


% \paragraph{Bounding spectral radius of $\M_i$}

\subsection{Generalization}
Here we generalize our result to a structural input distribution as 
\begin{align}
    \x = \U \v
\end{align}
where $\U$ is an orthogonal matrix and $\v$ is from a symmetric distribution, namely $\v_i$ is distributed as $-\v_i$. We will repeatly use the result of  












==> backup/relatedworks.tex <==
\section{Related works}
\cite{dieuleveut2017harder} has proved an improved convergence rate for averaged iterates of stochastic accelerated Nesterov when the covariance matrix is degenerated. In this case, they show that acceleration can improve $1/n$ convergence rate of SGD to $1/n^2$. When the matrix is not degenerated SGD can reach an exponential convergence rate $(1-c\mu/(L+\tr{\cov}))$ \cite{pillaud2017exponential,dieuleveut2017bridging} (we will prove this result later). \cite{jain2018accelerating} has shown that Nesterov's acceleration can improve the rate of SGD to $(1-\sqrt{\mu/(L}K)$. However, the constant $K$ in the rate can be larger than $\sqrt{\mu/L}$ in worst-cases. \cite{schmidt2018fast} has shown that accelerated stochastic gradient descent can obtain the square root improvement in the convergence rate for learning halfspace (which is a non-convex program). However, this result strongly rely on strong growth condition. The stochastic gradients satisfies strong grow condition if the following holds uniformly in $\w$: 
\begin{align} \label{assum:sgc}
    \E_\z  \left[ \| \nabla f_\z(\w) \|^2 \right] \leq \rho \| \nabla f(\w)\|^2 
\end{align}
Under the above assumption,~\cite{schmidt2018fast} show that a complicated update scheme over  3 sequences of iterates can reach to $1-\sqrt{\mu/(\rho^2L)}$ convergence rate. In the next lemma, we show that the constant $\rho$ can be as larger as $L/\mu$ for Gaussian inputs, hence their rate can is $1-(\mu/L)^{3/2}$ in worst case. This rate is worst than the rate for SGD. 
\begin{lemma}
    Consider the regression objective of Eq.~\ref{eq:f} on Gaussian input $\x \sim \N(0,\cov)$ and suppose that $y=0$. There exists a vector $\w_0 \in \R^d$ such that assumption~\ref{assum:sgc} does not hold for $\rho<L/\mu$. 
\end{lemma} 
\begin{proof} 
Let $\w_0$ be the eigenvector of $\cov$ associated with the smallest eigenvalue of $\cov$, i.e. ${\cov \w_0 = \mu \w_0}$. Then we use the result of lemma~\ref{lemma:gaussianity_consequence} to compute expected norm of stochastic gradients as 
\begin{align}
    \E \| \nabla f_\z(\w_0) \|^2 & = \w^\top_0 \E \left[ \x \x^\top \x \x^\top \right] \w_0 \\ 
    & \stackrel{\eqref{eq:gaussianity_consequence}}{=} \w_0^\top \cov^2 \w_0 + \tr[\cov]\w_0^\top \cov \w_0 \\ 
    & = \mu^2 + \tr[\cov] \mu \geq \mu (\mu+L)
\end{align}
The norm of gradient evaluated at $\w_0$ is 
\begin{align}
    \|\nabla f(\w) \|^2 = \w^\top_0 \cov^2 \w_0 = \mu^2
\end{align}
To satisfy assumption of Eq.~\eqref{assum:sgc}, we need to choose $\rho$ such that
\begin{align}
    \mu (\mu+L) \leq \rho \mu^2 \longleftarrow \rho \geq 1 + L/\mu. 
\end{align}
\end{proof}

==> non-realizable.tex <==
\section{Non-realizable cases} \label{sec:non_realizable}
 We shall now consider the question to what extent our results generalize to non-realizable cases where $f(\w_*) \neq 0$. Let vector $\v_k \in \R^{2d}$ be the concatenation of two consecutive iterates,  $\v_k:=[\w_{k+1},\w_k]$. Then the sequence $\{\v_k\}_{k=1}^n$ constitutes a Markov chain. The connection between stochastic optimization and Markov chains has been explored in \cite{dieuleveut2017bridging}. Theorem~\ref{thm:convergence_char} allows us to make a similar argument on this sequence of pairs of iterates. We follow the coupling approach proposed in \cite{dieuleveut2017bridging} by considering two coupling two sequences of iterates starting from different initial parameters: 
\begin{equation} \label{eq:coupling}
\begin{aligned}
    \w_{n+1} &= \w_n + \beta (\w_{n}-\w_{n-1}) - \gamma \nabla f_{\z_n}(\w_{n} + \alpha (\w_n - \w_{n-1})), \w_1 =\w_0 = \w \\ 
    \w_{n+1}'&= \w_n' + \beta (\w_{n}'-\w_{n-1}') - \gamma \nabla f_{\z_n}(\w_{n}' + \alpha (\w_n' - \w_{n-1}')), \w_1'= \w_0' = \w'
    \end{aligned}
\end{equation}
The two sequences are coupled via the shared random samples $\{\z_k\}_{k=1}^n$ in the above recurrences. For least-squares, it is easy to show that these sequences converges in a rate that is same as the convergence rate in realizable settings. The next lemma summarizes this results. 
\begin{lemma} [The forgetting speed in non-realizable cases] \label{lemma:forgetting}
    Consider the coupled sequences in Eq.~\eqref{eq:coupling} running on inputs following Assumption~\ref{assume:symmetric_inputs}. These sequence converges as
    \begin{align}
        \E \| \w'_{n} - \w_{n} \|^2 \leq 18 d^{3/2} \left(\| \C_{\Theta} \|_{\rho_\epsilon}\right)^{n+1}  \| \w' - \w \|^2/\epsilon
    \end{align}
    for all $\epsilon>0$ ($\C_{\Theta}$ is introduced in Eq.~\eqref{eq:cmatrix}). 
\end{lemma}

Appendix~\ref{sec:nonrealizable_app} presents the proof. The above results implies that the Markov chain $\{\v_k\}_{k=1}^n$ is stationary and forgetting its initial condition in rate $\bigo(\| \C_{\Theta} \|_{\rho_\epsilon}^n)$. This rate can be used to derive a composite rate for the convergence of tail-averaged iterates (i.e. bias-variance decomposition in \cite{dieuleveut2017harder}). For more details on the composite rate, we refer readers to Appendix~\ref{sec:nonrealizable_app}. 
 


